The Evolution of Emojis for Sharing Emotions: A Systematic Review of the HCI Literature

With the prevalence of instant messaging and social media platforms, emojis have become important artifacts for expressing emotions and feelings in our daily lives. We ask how HCI researchers have examined the role and evolution of emojis in sharing emotions over the past 10 years. We conducted a systematic literature review of papers addressing emojis employed for emotion communication between users. After screening more than 1,000 articles, we identified 42 articles of studies analyzing ways and systems that enable users to share emotions with emojis. Two main themes described how these papers have (1) improved how users select the right emoji from an increasing emoji lexicon, and (2) employed emojis in new ways and digital materials to enhance communication. We also discovered an increasingly broad scope of functionality across appearance, medium, and affordance. We discuss and offer insights into potential opportunities and challenges emojis will bring for HCI research.

==> discussion_notes.tex <==
%An important factor to consider is users' mental load [CITE]. Articles in the \textit{improvement} theme generally keep a familiar user experience. The improvements made were to address the increasing complexity of systems but not to allow them to be more customizable. The user is able to keep a similar mental model and enjoy only the benefits. This is in contrast to \textit{enhancement}, wherein the mental load is often proportional to the benefit added. A significant theme within this category is that of interpretability. The interpretability of messages sent with new technologies is a pertinent concern for users, and a cause of mental load - it often takes more effort to try and understand a deeper message than one that is sent with simply emojis. However, this mental load can also work in favor. For example, Auggie \cite{zhang_auggie_2022} is a system designed to take advantage of a message that intentionally takes more mental effort to create and experience. Though this may not end up being feasible for everyday lightweight communication, it serves to prove that mental load can be both a blessing and a curse.

%A forefront strength of the \textit{enhancement} category is to present unique ways to express oneself. The various implementations directly result in a more accessible and authentic experience for users. The new modalities of information being introduced also allows for users own meaning-making. We draw upon theories of self-presentation, which Goffman \cite{goffman_presentation_1959} refers to as 'conveying information about ourselves to others'. Recently, this theory has been applied to online personas in order to understand how people engage in self-reflection and presentation through social media and online communication. A more authentic perception of one's online presentation of self has been linked to higher self-esteem \cite{twomey_associations_2017} as well as increased well-being \cite{bij_de_vaate_how_2020}. 

%Scholars have theorized that just as emojis replaced emoticons, emojis are being replaced by new technology such as stickers \cite{konrad_sticker_2020, wang_more_2015}. However, such theories acknowledge that stickers have not achieved the widespread use that emojis have. While this may be attributed to the fact that stickers are newer, it may also be because of intrinsic differences.

%We see apps such as Snapchat providing Bitmojis, customizable avatars that can be seen in custom stickers between friends. We have Apple's Memoji, a 3-dimensional avatar that can even speak and emote in the user's voice. On Discord, users can upload custom images that can then be easily accessed as reactions or stickers within and across servers. All of this customization comes at the cost of user's data and privacy. 

%While all of the articles included in this review presented emotion communication research, many articles may not seem related to emojis. However, we argue that while the work it represents do not fit the traditional definition of emojis as \emph{`picture characters`}, they do fulfill the same roles. Emoji has long been used as a marker for emotion communication, typically in conjunction with other forms of messaging such as text. With innovations to communication outside of textual media, emojis as a textual icon do not see use anymore. However, this does not mean that the role of emojis has disappeared. The design of emotion communication methods in media is still necessary. In this light, we argue that the articles selected for this literature review all propose emoji-related research work, either by way of directly relating to emojis or by relating in the same purpose of emoji as emotion communication tools. Since there is no simple word to describe this type of work, for simplicity we refer to all these works that deal with emotion communication as emoji related works. %%redo

There is an increasing demand for greater customization within the major communication providers. As platforms increase in complexity and richness, they trigger new efforts to make emoji that can keep up with these platforms. As users enjoy these features, companies are motivated to create more function, thus creating a feedback loop that drives the evolution towards more information-carrying features. As this feedback loop continues, emoji development will continue towards greater customization and complexity as evidenced by current research.

%this part is just thoughts and general ideas to flesh out later
%Similarly, emotion communication based on biosignals can unintentionally convey information. Firstly, the sensing and interpreting of biosignals as emotion can be inaccurate for the same reasons that polygraph tests are not admissible as evidence in American courts of law. When you can see someone else's interpreted biosignal information, you are relying on a machine model to read their emotion, thus adding a layer of obfuscation between yourself and your communicator. 

%Secondly, the biosignal communication may be unwanted. If a user is feeling negative emotions, then they may not want to portray those emotions to other users. If they wish to hide their emotional state by turning off their biosignal sensing device, the lack of information being sent can also be a message to other users that they are trying to hide. In this case, simply opting into using this means of communication is similar to signing a social contract towards always showing their emotional state.


%% different forms of emojis currently
% can also talk about customization and complexity increasing, whether customization will continue to increase and whether complexity will plateau or simply increase exponentially with customization reaching a limit?

%edits
%Emojis and the way we use them  encodes our data. This includes information such as self-presentation as well as interpersonal relationships.

%The increasingly personalized and emotional experiences that many of the researchers seek to provide hinge upon users sharing more about themselves with each other, and by medium, the system that they are using. These systems typically acknowledge privacy concerns by stating that they do not record photos, messages, or other sensitive information in their databases. 

% however, these systems want you to share more information - their goal is to improve communication, which, the definition being, being able to convey more completely and accurate to the message author's original intention is. In real life, this is not perfect. Nonverbal cues can be both intentional and unintentional, conveying or betraying the author's true intentions. for example, biosignal based communication methods 

%Within our literature review, we discovered a trend of divergence in the research being done on emojis. Though emojis are incredibly prevalent in everyday use and a staple of popular culture, with their own contextual and community-assigned meanings, the community seems split on whether emojis are sufficient emotion communication markers for the future of communication.

